Catalight -- an open source automated photocatalytic reactor package illustrated through plasmonic acetylene hydrogenation

An open-source and modular Python package, Catalight, is developed and demonstrated to automate (photo)catalysis measurements. (Photo)catalysis experiments require studying several parameters to evaluate performance, including temperature, gas flow rate and composition, illumination power, and spectral profile. Catalight orchestrates measurements over this complicated parameter space and systematically stores, analyzes, and visualizes the resulting data. To showcase the capabilities of Catalight, we perform an automated apparent activation barrier measurement of acetylene hydrogenation over a plasmonic AuPd catalyst on Al2O3 support, simultaneously varying laser power, wavelength, and temperature in a multi-day experiment controlled by a simple Python script. Our chemical results unexpectedly show an increased activation barrier upon light excitation, contrary to previous findings for other plasmonic reactions and catalysts. We show that the reaction rate order with respect to both acetylene and hydrogen is unchanged upon illumination, suggesting that molecular surface coverage is not changing under light excitation. By analyzing the inhomogeneity of the laser induced heating, we attribute these results to a partial photothermal effect combined with a photochemical/hot electron driven mechanism. Our findings highlight the capabilities of a new experiment automation tool; explore the photocatalytic mechanism for an industrially relevant reaction; and identify systematic sources of error in canon photocatalysis experimental procedures.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}


# Uncomment this line to compile the differences in the SI
#  $pdflatex = "latexdiff SI_v3.tex SI_v4.tex > main-d.tex; pdflatex %O  main-d"


# Uncomment this line to compile the differences in the main text
# $pdflatex = "latexdiff Main_v3.tex Main_v4.tex > main-d.tex; pdflatex %O  main-d"
